Anomaly Detection on X-Rays Using Self-Supervised Aggregation Learning

Deep anomaly detection models using a supervised mode of learning usually work under a closed set assumption and suffer from overfitting to previously seen rare anomalies at training, which hinders their applicability in a real scenario. In addition, obtaining annotations for X-rays is very time consuming and requires extensive training of radiologists. Hence, training anomaly detection in a fully unsupervised or self-supervised fashion would be advantageous, allowing a significant reduction of time spent on the report by radiologists. In this paper, we present SALAD, an end-to-end deep self-supervised methodology for anomaly detection on X-Ray images. The proposed method is based on an optimization strategy in which a deep neural network is encouraged to represent prototypical local patterns of the normal data in the embedding space. During training, we record the prototypical patterns of normal training samples via a memory bank. Our anomaly score is then derived by measuring similarity to a weighted combination of normal prototypical patterns within a memory bank without using any anomalous patterns. We present extensive experiments on the challenging NIH Chest X-rays and MURA dataset, which indicate that our algorithm improves state-of-the-art methods by a wide margin.

==> related_work.tex <==
\section{Related Work}
Classical anomaly detection (AD) methods such as the One-Class SVM (OC-SVM) \cite{scholkopf2001}, Local Outlier Factor \cite{breunig2000lof}, or Isolation Forest \cite{liu2008isolation} often fail to be effective on high-dimensional data or be scaled to large datasets.  To alleviate this concern, state-of-the-art methods like Deep SVDD \cite{ruff2018deep} and Deep SAD \cite{ruff2019deep} consider to learn deep CNN features as an alternative for classifical one-class anomaly detection.

